On Tackling Explanation Redundancy in Decision Trees

Decision trees (DTs) epitomize the ideal of interpretability of machine learning (ML) models. The interpretability of decision trees motivates explainability approaches by so-called intrinsic interpretability, and it is at the core of recent proposals for applying interpretable ML models in high-risk applications. The belief in DT interpretability is justified by the fact that explanations for DT predictions are generally expected to be succinct. Indeed, in the case of DTs, explanations correspond to DT paths. Since decision trees are ideally shallow, and so paths contain far fewer features than the total number of features, explanations in DTs are expected to be succinct, and hence interpretable. This paper offers both theoretical and experimental arguments demonstrating that, as long as interpretability of decision trees equates with succinctness of explanations, then decision trees ought not be deemed interpretable. The paper introduces logically rigorous path explanations and path explanation redundancy, and proves that there exist functions for which decision trees must exhibit paths with arbitrarily large explanation redundancy. The paper also proves that only a very restricted class of functions can be represented with DTs that exhibit no explanation redundancy. In addition, the paper includes experimental results substantiating that path explanation redundancy is observed ubiquitously in decision trees, including those obtained using different tree learning algorithms, but also in a wide range of publicly available decision trees. The paper also proposes polynomial-time algorithms for eliminating path explanation redundancy, which in practice require negligible time to compute. Thus, these algorithms serve to indirectly attain irreducible, and so succinct, explanations for decision trees.

==> runex/runex05.tex <==

\begin{exmp} \label{ex:runex05}
  The third running example is shown in~\cref{fig:runex05}. In
  contrast with the first two examples, one produced with well-known
  DT learning algorithms and the second one produced with a tool
  offering guarantees of optimality and sparseness, this third example
  is handmade. It shows an hypothetical decision tree for predicting
  bank loan default, and will serve to illustrate specific aspects
  (e.g.\ multi-valued features) of the ideas proposed in the paper,
  and which are not covered by the first two running examples.
\end{exmp}
%
\begin{figure}[t]
  \begin{subfigure}{\textwidth}
    \begin{center}
      \scalebox{0.925}{\input{./tables/bankdef}}
    \end{center}
    \caption{Problem definition}
  \end{subfigure}
  \begin{subfigure}{\textwidth}
    \begin{center}
      \scalebox{0.925}{\input{./texfigs/tree08}}
    \end{center}
    \caption{Decision tree}
  \end{subfigure}
  \caption{Third running example}
  \label{fig:runex05}
\end{figure}


==> tables/bankdef.tex <==
\renewcommand{\arraystretch}{1.05}
%\renewcommand{\tabcolsep}{0.5em}
\begin{tabular}{ccccc}
  \toprule
  \multicolumn{5}{c}{Bank loan default, with $\mbf{x}=(E,M,S,A)$ and $\fml{K}=\{\clyes,\clnot\}$}\\
  %
  \toprule
  Feature & ID & Var. & Domain & Coded Domain \\
  \toprule
  Ethnic Group & 1 & $E$ & $\{\tn{European},\tn{African},\tn{Asian}\}$ &
  $\{E_1,E_2,E_3\}$ \\
  %\hline
  Value of Mortgage & 2 & $M$ &
  $\{{\le}\,100\tn{K},{>}\,100\tn{K}\}$ & $\{M_1,M_2\}$ \\
  %\hline
  Salary of Applicant & 3 & $S$ &
  $\{{\le}\,20\tn{K},{>}\,20\tn{K}\land{\le}\,50\tn{K},{>}\,50\tn{K}\}$ &
  $\{S_1,S_2,S_3\}$ \\
  %\hline
  Age of Applicant & 4 & $A$ & $\{{\le}\,40,{>}\,40\land{\le}\,55,{>}\,55\}$ &
  $\{A_1,A_2,A_3\}$ \\
  \bottomrule
\end{tabular}


==> tables/osdt-tab01.tex <==
%
\renewcommand{\tabcolsep}{0.35em}
\renewcommand{\arraystretch}{1.0875}
\begin{tabular}{|ccc|c|} \hline%\toprule
  \multicolumn{4}{|c|}{$\tn{BR}=1,\tn{TR}=1$}
  \\ \hline%\midrule
  %\toprule
  MM & BL & TL &
  %$\kappa(\tn{MM},\tn{BR},\tn{TR},\tn{BL},\tn{TL})$ \\
  $\kappa(\cdot)$ \\
  \hline%\midrule%\toprule
  %1  &  1 &
  0 & 0  & 0  & 1 \\
  %1  &  1 &
  0 & 0  & 1  & 1 \\
  %1  &  1 &
  0 & 1  & 0  & 1 \\
  %1  &  1 &
  0 & 1  & 1  & 1 \\
  %1  &  1 &
  1 & 0  & 0  & 1 \\
  %1  &  1 &
  1 & 0  & 1  & 1 \\
  %1  &  1 &
  1 & 1  & 0  & 1 \\
  %1  &  1 &
  1 & 1  & 1  & 1 \\
  \hline%\bottomrule
\end{tabular}
%


==> tables/osdt-tab02.tex <==
\renewcommand{\tabcolsep}{0.35em}
\renewcommand{\arraystretch}{1.0875}
\begin{tabular}{|c|c|c|} \hline
  $\tn{middle-middle}=\tn{x}\:\tn{iff}\:\tn{MM}=1$
  &
  $\tn{top-left}=\tn{x}\:\tn{iff}\:\tn{TL}=1$
  &
  \\ \hline
  $\tn{bottom-right}=\tn{x}\:\tn{iff}\:\tn{BR}=1$
  &
  $\tn{bottom-left}=\tn{x}\:\tn{iff}\:\tn{BL}=1$
  &
  $\tn{top-right}=\tn{x}\:\tn{iff}\:\tn{TR}=1$
  \\ \hline
\end{tabular} 


==> tables/tab-inst.tex <==
\setlength{\tabcolsep}{5pt}
\let\lpr\undefined
\let\rpr\undefined
\newcommand{\lpr}{(}
\newcommand{\rpr}{)}

\begin{table}[t] %h
\centering
\resizebox{0.65\textwidth}{!}{
  \begin{tabular}{l r c c c c S[table-format=2.0] cccc}
\toprule[1.2pt]
\multirow{2}{*}{\bf Dataset} & \multirow{2}{*}{\bf Instance} & \multicolumn{3}{c}{\bf DT} & \multicolumn{5}{c}{\bf AXp} \\
\cmidrule[0.8pt](lr{.75em}){3-5}
\cmidrule[0.8pt](lr{.75em}){6-10}
&  & {\bf D} & {\bf \#N} & {\bf \%A} & {\bf P} &  {\bf m} & {\bf M}  & {\bf avg} & {\bf n}  \\
\toprule[1.2pt]

%%adult & adult\_0 & 17 & 509 & 73 & 11 & 6 & 6 & 6 & 4  \\
%adult & adult\_1 & 17 & 509 & 73 & 11  & 5 & 6 & 5.8 & 12\\
\multirow{3}{*}{adult} & adult\_015 & \multirow{3}{*}{17} & \multirow{3}{*}{509} & \multirow{3}{*}{73} & 16 & 8 & 8 & 8 & 2 \\
 & adult\_089 &  &  &  & 14 & 5 & 6 & 5.5 & 2 \\
 & adult\_190 &  &  &  & 16 & 5 & 5 & 5 & 1 \\
%adult & adult\_278 & 17 & 509 & 73 & 17 & 7 & 7 & 7 & 2 \\

\midrule

\multirow{3}{*}{allhyper} & allhyper\_0 &  \multirow{3}{*}{14} &  \multirow{3}{*}{49} & \multirow{3}{*}{96} & 14 & 4 &  5 & 4.6 & 6 \\ 
 & allhyper\_1 &   &  &  & 9 & 4 &  5 & 4.5 & 8 \\ 
 & allhyper\_4 &  &   &  & 14 & 4 &  5 & 4.6 & 6 \\ 
	 
\midrule	 


\multirow{3}{*}{ann-thyroid} &  ann-thyroid\_3 &  \multirow{3}{*}{48} & \multirow{3}{*}{222} & \multirow{3}{*}{93} & 40 & 5 & 6 & 5.6 & 3 \\
 &  ann-thyroid\_4 &   &  &  & 36 & 5 & 6 & 5.6 & 3 \\
 &  ann-thyroid\_7 &   &  &  & 20 & 5 & 6 & 5.5 & 2 \\

\midrule

\multirow{3}{*}{coil2000} & coil2000\_045 &  \multirow{3}{*}{12} & \multirow{3}{*}{177} & \multirow{3}{*}{91} & 10 &  2 & 4 & 3.8 & 39 \\
 & coil2000\_218 &   &  &  & 10 &  2 & 4 & 3.8 & 39 \\
 & coil2000\_244 &   &  &  & 10 &  2 & 4 & 3.8 & 30 \\

%\midrule
%connect-4 & 22 & 9089 & 75 & 

\midrule

\multirow{3}{*}{fars} &  fars\_002 & \multirow{3}{*}{60} & \multirow{3}{*}{9969} & \multirow{3}{*}{76} & 29 & 11 & 11 & 11 & 2 \\
%fars &  fars\_3 & 60 & 9969 & 76 & 25 & 8 & 13 & 11 & 3 \\
%fars &  fars\_18 & 60 & 9969 & 76 & 18 & 8 & 8 & 8 & 1 \\
%fars &  fars\_66 & 60 & 9969 & 76 & 52 & 13 & 14 & 13.5 & 2 \\
 &  fars\_125 &  &  &  & 42 & 10 & 14 & 12.3 & 9 \\
 &  fars\_354 &  &  &  & 48 & 9 & 9 & 9 & 1 \\

\midrule

\multirow{3}{*}{kddcup} & kddcup\_01 & \multirow{3}{*}{29} & \multirow{3}{*}{269} & \multirow{3}{*}{99} &  23  & 11 & 12 & 11.5 & 16\\
 & kddcup\_02 &  &  &  &  23  & 11 & 12 & 11.5 & 16\\
%kddcup & kddcup\_3 & 29 & 269 & 99 &  23  & 11 & 12 & 11.5 & 16\\
 & kddcup\_21 &  &  &  &  27 & 12 & 13 & 12.5 & 8 \\
%kddcup & kddcup\_24 & 29 & 269 & 99 &  24  & 11 & 11 & 11 & 2\\

\bottomrule[1.2pt]
\end{tabular}
}
\caption{\footnotesize{
    Samples of 6 real-world datasets highlighting computed 
    instance-based AXp's in DTs learned with ITI, that require
    deep trees.
    % 
    For each dataset, the table displays 3 tested instances. 
    %
    Columns  {\bf D}, {\bf \#N} and {\bf \%A}  denote,
    resp.\, depth, number of nodes and accuracy of trained DT
    with ITI tool. 
    %
    Next, column  {\bf P} reports the consistent
    path's length in the DT with the input instance. 
    %
    Then, the average (min. or max., resp.) length of the computed 
    path-restricted AXp's given the input instance, is denoted by 
    {\bf avg} ({\bf m} and {\bf M}, resp.).
    % 
    Finally, the total number of AXp's is shown in  column {\bf n}.
    }
 } \label{tab:inst}
\end{table}


==> tables/tab-res.tex <==
\setlength{\tabcolsep}{4pt}
\let\lpr\undefined
\let\rpr\undefined
\newcommand{\lpr}{(}
\newcommand{\rpr}{)}


%\begin{table}[htb]
%\centering
%\Rotatebox{90}{%
\begin{table}[t] %h!
  \begin{adjustbox}{addcode={\begin{minipage}{\width}}{\caption{%
     \footnotesize{Path explanation redundancy in decision trees
    obtained with IAI and ITI.
    %
    The table shows tree statistics for IAI and ITI, namely, tree
    depth {\bf D}, number of nodes {\bf \#N}, test accuracy {\bf \%A}
    and number of paths {\bf \#P}.
    %
    The percentage of explanation-redundant paths (XRP's) is given as {\bf \%R}
    while the percentage of data instances (measured for the \emph{entire}
    feature space) covered by XRP's is {\bf \%C}.
    %
    Focusing solely on the XRP's, the average (min.~or max., resp.)
    percentage of explanation-redundant features per path is denoted 
    by {\bf \%avg}  ({\bf \%m} and {\bf \%M}, resp.). }
  }\label{tab:res}\end{minipage}},rotate=90,center}

\resizebox{0.75\textheight}{!}{
  \begin{tabular}{lcS[table-format=3.0]S[table-format=3.0]S[table-format=2.0]S[table-format=2.0]S[table-format=2.0]cccS[table-format=2.0]S[table-format=4.0]S[table-format=3.0]S[table-format=4.0]S[table-format=2.0]S[table-format=2.0]S[table-format=2.0]cS[table-format=2.0]}
\toprule[1.2pt]
\multirow{2}{*}{\bf Dataset} & \multicolumn{9}{c}{\bf IAI} & \multicolumn{9}{c}{\bf ITI} \\
  \cmidrule[0.8pt](lr{.75em}){2-10}
  \cmidrule[0.8pt](lr{.75em}){11-19}
&  {\bf D} & {\bf \#N} & {\bf \%A} & {\bf \#P} & {\bf \%R} & {\bf \%C} & {\bf \%m} & {\bf \%M} & {\bf \%avg} & {\bf D} & {\bf \#N} & {\bf \%A} & {\bf \#P} & {\bf \%R} & {\bf \%C} & {\bf \%m} & {\bf \%M} & {\bf \%avg} \\
\toprule[1.2pt]


adult &  6 & 83 & 78 & 42 & 33 & 25 & 20 & 40 & 25 & 17 & 509 &  73 & 255 & 75 & 91 & 10 & 66 & 22  \\
ann-thyroid & 6 & 61 & 97 & 31 & 25 & 30 & 20 & 50 & 36 & 48 & 223 & 93 & 112 & 65 & 46 & 11 & 75 & 22 \\
anneal &  6 & 29 & 99 & 15 & 26 & 16 & 16 & 33 & 21 & 9 & 31 &  100 & 16 & 25 & 4 & 12 & 20 & 16  \\
backache  & 4 & 17 & 72 & 9 & 33 & 39 & 25 & 33 & 30 & 3 & 9 &  91 & 5 & 80 & 87 & 50 & 66 & 54  \\
bank  & 6 & 113 & 88 & 57 & 5 & 12 & 16 & 20 & 18 & 19 & 1467 &  86 & 734 & 69 & 64 & 7 & 63 & 27  \\
biodegradation  & 5 & 19 & 65 & 10 & 30 & 1 & 25 & 50 & 33 & 8 & 71 &  76 & 36 & 50 & 8 & 14 & 40 & 21  \\
cancer & 6 & 37 & 87 & 19 & 36 & 9 & 20 & 25 & 21 & 5 & 21 &  84 & 11 & 54 & 10 & 25 & 50 & 37  \\
car  & 6 & 43 & 96 & 22 & 86 & 89 & 20 & 80 & 45 & 11 & 57 &  98 & 29 & 65 & 41 & 16 & 50 & 30  \\
colic  & 6 & 55 & 81 & 28 & 46 & 6 & 16 & 33 & 20 & 4 & 17 &  80 & 9 & 33 & 27 & 25 & 25 & 25  \\
compas  & 6 & 77 & 34 & 39 & 17 & 8 & 16 & 20 & 17 & 15 & 183 &  37 & 92 & 66 & 43 & 12 & 60 & 27  \\
contraceptive  & 6 & 99 & 49 & 50 & 8 & 2 & 20 & 60 & 37 & 17 & 385 &  48 & 193 & 27 & 32 & 12 & 66 & 21  \\
dermatology  & 6 & 33 & 90 & 17 & 23 & 3 & 16 & 33 & 21 & 7 & 17 &  95 & 9 & 22 & 0 & 14 & 20 & 17  \\
divorce  & 5 & 15 & 90 & 8 & 50 & 19 & 20 & 33 & 24 & 2 & 5 &  96 & 3 & 33 & 16 & 50 & 50 & 50  \\
german  & 6 & 25 & 61 & 13 & 38 & 10 & 20 & 40 & 29 & 10 & 99 &  72 & 50 & 46 & 13 & 12 & 40 & 22  \\
heart-c  & 6 & 43 & 65 & 22 & 36 & 18 & 20 & 33 & 22 & 4 & 15 &  75 & 8 & 87 & 81 & 25 & 50 & 34  \\
heart-h  & 6 & 37 & 59 & 19 & 31 & 4 & 20 & 40 & 24 & 8 & 25 &  77 & 13 & 61 & 60 & 20 & 50 & 32  \\
kr-vs-kp  & 6 & 49 & 96 & 25 & 80 & 75 & 16 & 60 & 33 & 13 & 67 &  99 & 34 & 79 & 43 & 7 & 70 & 35  \\
lending  & 6 & 45 & 73 & 23 & 73 & 80 & 16 & 50 & 25 & 14 & 507 &  65 & 254 & 69 & 80 & 12 & 75 & 25  \\
letter  & 6 & 127 & 58 & 64 & 1 & 0 & 20 & 20 & 20 & 46 & 4857 &  68 & 2429 & 6 & 7 & 6 & 25 & 9  \\
lymphography  & 6 & 61 & 76 & 31 & 35 & 25 & 16 & 33 & 21 & 6 & 21 &  86 & 11 & 9 & 0 & 16 & 16 & 16  \\
mushroom  & 6 & 39 & 100 & 20 & 80 & 44 & 16 & 33 & 24 & 5 & 23 &  100 & 12 & 50 & 31 & 20 & 40 & 25  \\
pendigits  & 6 & 121 & 88 & 61 & 0 & 0 & \textemdash & \textemdash & \textemdash & 38 & 937 &  85 & 469 & 25 & 86 & 6 & 25 & 11  \\
promoters  & 1 & 3 & 90 & 2 & 0 & 0 & \textemdash & \textemdash & \textemdash & 3 & 9 &  81 & 5 & 20 & 14 & 33 & 33 & 33  \\
recidivism & 6 & 105 & 61 & 53 & 28 & 22 & 16 & 33 & 18 & 15 & 611 &  51 & 306 & 53 & 38 & 9 & 44 & 16  \\
seismic\_bumps  & 6 & 37 & 89 & 19 & 42 & 19 & 20 & 33 & 24 & 8 & 39 &  93 & 20 & 60 & 79 & 20 & 60 & 42  \\
shuttle & 6 & 63 & 99 & 32 & 28 & 7 & 20 & 33 & 23 & 23 & 159 &  99 & 80 & 33 & 9 & 14 & 50 & 30  \\
soybean & 6 & 63 & 88 & 32 & 9 & 5 & 25 & 25 & 25 & 16 & 71 &  89 & 36 & 22 & 1 & 9 & 12 & 10  \\
spambase  & 6 & 63 & 75 & 32 & 37 & 12 & 16 & 33 & 19 & 15 & 143 &  91 & 72 & 76 & 98 & 7 & 58 & 25  \\
spect & 6 & 45 & 82 & 23 & 60 & 51 & 20 & 50 & 35 & 6 & 15 &  86 & 8 & 87 & 98 & 50 & 83 & 65  \\
splice  & 3 & 7 & 50 & 4 & 0 & 0 & \textemdash & \textemdash & \textemdash & 88 & 177 &  55 & 89 & 0 & 0 & \textemdash & \textemdash & \textemdash  \\


\bottomrule[1.2pt]
\end{tabular}
}
\end{adjustbox}
%}
%\caption{
 % \footnotesize{Path explanation redundancy in decision trees
 %   obtained with IAI and ITI.
 %   %
 %   %Columns {\bf D}, {\bf \#N}, {\bf \#P}, {\bf \%R}, {\bf
 %   %   \%C}, {\bf \%m}, {\bf \%M} and  {\bf \%avg} have the same
 %   %meaning as in~\autoref{tab:dtrees}.
 %   %
 %   The table shows tree statistics for IAI and ITI, namely, tree
 %   depth {\bf D}, number of nodes {\bf \#N}, test accuracy {\bf \%A}
 %   and number of paths {\bf \#P}.
 %   %
 %   The percentage of explanation-redundant paths (XRP's) is given as {\bf \%R}
 %   while the percentage of data instances (measured for the \emph{entire}
 %   feature space) covered by XRP's is {\bf \%C}.
 %   %
 %   Focusing solely on the XRP's, a single
 %   AXp is extracted and the average (min.~or max., resp.)
 %   percentage of explanation redundant features per path is denoted 
 %   by {\bf \%avg}  ({\bf \%m} and {\bf \%M}, resp.).
 % }
  %
 % \label{tab:res}
%}
\end{table}


%%======================================================================%%



==> tables/tab-runtime.tex <==
\setlength{\tabcolsep}{4pt}
\let\lpr\undefined
\let\rpr\undefined
\newcommand{\lpr}{(}
\newcommand{\rpr}{)}

\begin{table}[t] %h!
  \begin{adjustbox}{addcode={\begin{minipage}{\width}}{\caption{%
   \footnotesize{Assessing runtimes of the tree traversal
    algorithm and the propositional horn encoding approach for
    extracting one AXp.
    %
    The table reports the results for DTs trained with ITI and IAI
    learning tools. Columns  {\bf m}, {\bf M} and  {\bf avg}  report,
    resp.\ , the minimal, maximal and average runtime (in second)
    to compute an AXp, while column {\bf Tot} reports the total
    runtime (in second) of all tested instances in a dataset. } 
  }\label{tab:runtime}\end{minipage}},rotate=90,center}
  
\resizebox{0.75\textheight}{!}{
  \begin{tabular}{l cccc cccc cccc cccc}
\toprule[1.2pt]
\multirow{3}{*}{\bf Dataset}  & \multicolumn{8}{c}{\bf IAI} & \multicolumn{8}{c}{\bf ITI} \\
\cmidrule[0.8pt](lr{.75em}){2-9}
\cmidrule[0.8pt](lr{.75em}){10-17}
& \multicolumn{4}{c}{\bf Traversal}  & \multicolumn{4}{c}{\bf Horn}   & \multicolumn{4}{c}{\bf Traversal}  & \multicolumn{4}{c}{\bf Horn} \\  
\cmidrule[0.8pt](lr{.75em}){2-5}
\cmidrule[0.8pt](lr{.75em}){6-9}
\cmidrule[0.8pt](lr{.75em}){10-13}
\cmidrule[0.8pt](lr{.75em}){14-17}
&  {\bf m} & {\bf M} & {\bf avg} & {\bf Tot} & {\bf m} & {\bf M}  & {\bf avg} & {\bf Tot} & {\bf m} & {\bf M}  & {\bf avg} & {\bf Tot} & {\bf m} & {\bf M}  & {\bf avg} & {\bf Tot} \\
\toprule[1.2pt]

%IndiansDiabetes & 0.001 & 0.003 & 0.001 & 0.73 & 0.001 & 0.002 & 0.001 & 0.63 & 0.001 & 0.003 & 0.002 & 1.19 & 0.001 & 0.002 & 0.001 & 1.02 \\
adult & 0.001 & 0.059 & 0.002 & 3.52 & 0.001 & 0.005 & 0.002 & 2.93 & 0.004 & 0.038 & 0.007 & 12.89 & 0.008 & 0.036 & 0.010 & 19.00 \\
%allhyper & 0.001 & 0.006 & 0.002 & 1.88 & 0.001 & 0.005 & 0.001 & 1.23 & 0.001 & 0.004 & 0.002 & 2.39 & 0.001 & 0.002 & 0.001 & 1.20 \\
ann-thyroid & 0.001 & 0.005 & 0.002 & 3.67 & 0.001 & 0.005 & 0.001 & 2.85 & 0.002 & 0.041 & 0.006 & 12.14 & 0.004 & 0.029 & 0.005 & 9.64 \\
anneal & 0.001 & 0.005 & 0.001 & 1.22 & 0.001 & 0.003 & 0.001 & 0.75 & 0.001 & 0.006 & 0.001 & 0.96 & 0.001 & 0.004 & 0.001 & 0.70 \\
%appendicitis & 0.000 & 0.000 & 0.000 & 0.029 & 0.000 & 0.000 & 0.000 & 0.032 & 0.000 & 0.001 & 0.000 & 0.028 & 0.000 & 0.001 & 0.000 & 0.033 \\
%australian & 0.001 & 0.003 & 0.001 & 0.93 & 0.001 & 0.002 & 0.001 & 0.71 & 0.001 & 0.004 & 0.001 & 0.94 & 0.001 & 0.002 & 0.001 & 0.61 \\
%auto & 0.001 & 0.005 & 0.001 & 0.22 & 0.001 & 0.005 & 0.001 & 0.18 & 0.001 & 0.005 & 0.002 & 0.33 & 0.001 & 0.005 & 0.001 & 0.24 \\
backache & 0.001 & 0.001 & 0.001 & 0.13 & 0.000 & 0.001 & 0.001 & 0.094 & 0.000 & 0.001 & 0.000 & 0.077 & 0.000 & 0.001 & 0.000 & 0.065 \\
%balance & 0.001 & 0.004 & 0.001 & 0.82 & 0.002 & 0.005 & 0.002 & 1.15 & 0.001 & 0.057 & 0.001 & 0.86 & 0.002 & 0.006 & 0.002 & 1.23 \\
bank & 0.002 & 0.062 & 0.003 & 34.45 & 0.002 & 0.008 & 0.002 & 25.53 & 0.013 & 0.090 & 0.027 & 19.64 & 0.025 & 0.092 & 0.033 & 24.21 \\
%banknote & 0.000 & 0.001 & 0.000 & 0.12 & 0.000 & 0.001 & 0.000 & 0.14 & 0.001 & 0.002 & 0.001 & 0.47 & 0.001 & 0.003 & 0.001 & 0.54 \\
biodegradation & 0.000 & 0.003 & 0.001 & 0.21 & 0.000 & 0.002 & 0.001 & 0.18 & 0.002 & 0.007 & 0.003 & 0.98 & 0.001 & 0.003 & 0.002 & 0.48 \\
%biomed & 0.000 & 0.001 & 0.000 & 0.064 & 0.000 & 0.001 & 0.000 & 0.073 & 0.001 & 0.002 & 0.001 & 0.17 & 0.001 & 0.001 & 0.001 & 0.16 \\
%breast-cancer & 0.001 & 0.003 & 0.002 & 0.42 & 0.001 & 0.004 & 0.001 & 0.35 & 0.000 & 0.001 & 0.001 & 0.19 & 0.001 & 0.001 & 0.001 & 0.17 \\
%bupa & 0.001 & 0.003 & 0.001 & 0.33 & 0.001 & 0.002 & 0.001 & 0.34 & 0.001 & 0.002 & 0.001 & 0.33 & 0.001 & 0.005 & 0.001 & 0.35 \\
cancer & 0.001 & 0.003 & 0.001 & 0.53 & 0.001 & 0.003 & 0.001 & 0.39 & 0.001 & 0.004 & 0.001 & 0.32 & 0.001 & 0.002 & 0.001 & 0.26 \\
car & 0.001 & 0.004 & 0.001 & 0.52 & 0.001 & 0.002 & 0.001 & 0.48 & 0.001 & 0.002 & 0.001 & 0.47 & 0.001 & 0.002 & 0.001 & 0.59 \\
%cleveland & 0.001 & 0.005 & 0.001 & 0.25 & 0.001 & 0.004 & 0.002 & 0.31 & 0.001 & 0.002 & 0.001 & 0.23 & 0.001 & 0.002 & 0.001 & 0.25 \\
%coil2000 & 0.003 & 0.036 & 0.009 & 21.56 & 0.002 & 0.009 & 0.002 & 5.77 & 0.004 & 0.044 & 0.018 & 44.26 & 0.003 & 0.029 & 0.004 & 11.02 \\
colic & 0.001 & 0.005 & 0.002 & 0.71 & 0.001 & 0.002 & 0.001 & 0.43 & 0.000 & 0.001 & 0.001 & 0.24 & 0.000 & 0.001 & 0.000 & 0.18 \\
compas & 0.001 & 0.004 & 0.002 & 0.66 & 0.001 & 0.004 & 0.002 & 0.52 & 0.002 & 0.065 & 0.004 & 1.37 & 0.003 & 0.005 & 0.004 & 1.28 \\
contraceptive & 0.001 & 0.005 & 0.002 & 0.70 & 0.002 & 0.004 & 0.002 & 0.78 & 0.003 & 0.064 & 0.006 & 2.64 & 0.006 & 0.012 & 0.007 & 2.87 \\
dermatology & 0.001 & 0.005 & 0.001 & 0.50 & 0.001 & 0.002 & 0.001 & 0.31 & 0.000 & 0.001 & 0.001 & 0.27 & 0.000 & 0.001 & 0.001 & 0.19 \\
divorce & 0.000 & 0.002 & 0.001 & 0.10 & 0.000 & 0.001 & 0.001 & 0.076 & 0.000 & 0.001 & 0.000 & 0.033 & 0.000 & 0.002 & 0.000 & 0.041 \\
%ecoli & 0.001 & 0.003 & 0.001 & 0.25 & 0.001 & 0.002 & 0.001 & 0.32 & 0.001 & 0.057 & 0.001 & 0.46 & 0.002 & 0.004 & 0.002 & 0.62 \\
%fars & 0.001 & 0.004 & 0.002 & 3.26 & 0.001 & 0.004 & 0.002 & 2.86 & 0.066 & 0.18 & 0.093 & 172.34 & 0.19 & 0.32 & 0.20 & 374.52 \\
german & 0.001 & 0.004 & 0.001 & 0.76 & 0.001 & 0.002 & 0.001 & 0.65 & 0.002 & 0.007 & 0.003 & 3.19 & 0.002 & 0.003 & 0.002 & 2.03 \\
heart-c & 0.001 & 0.003 & 0.001 & 0.42 & 0.001 & 0.003 & 0.001 & 0.30 & 0.000 & 0.001 & 0.001 & 0.17 & 0.000 & 0.001 & 0.000 & 0.14 \\
heart-h & 0.001 & 0.004 & 0.001 & 0.39 & 0.001 & 0.005 & 0.001 & 0.27 & 0.001 & 0.001 & 0.001 & 0.21 & 0.001 & 0.001 & 0.001 & 0.18 \\
%heart-statlog & 0.001 & 0.003 & 0.001 & 0.26 & 0.001 & 0.002 & 0.001 & 0.23 & 0.000 & 0.001 & 0.001 & 0.14 & 0.000 & 0.001 & 0.000 & 0.11 \\
%hepatitis & 0.001 & 0.002 & 0.001 & 0.12 & 0.000 & 0.002 & 0.001 & 0.084 & 0.000 & 0.001 & 0.000 & 0.064 & 0.000 & 0.002 & 0.000 & 0.062 \\
%house-votes-84 & 0.001 & 0.006 & 0.002 & 0.56 & 0.001 & 0.002 & 0.001 & 0.32 & 0.000 & 0.000 & 0.000 & 0.10 & 0.000 & 0.001 & 0.000 & 0.100 \\
%hungarian & 0.001 & 0.003 & 0.001 & 0.27 & 0.001 & 0.005 & 0.001 & 0.24 & 0.001 & 0.002 & 0.001 & 0.23 & 0.000 & 0.002 & 0.001 & 0.18 \\
%ionosphere & 0.000 & 0.001 & 0.000 & 0.15 & 0.000 & 0.002 & 0.001 & 0.18 & 0.001 & 0.003 & 0.001 & 0.36 & 0.000 & 0.002 & 0.001 & 0.26 \\
%iris & 0.000 & 0.003 & 0.001 & 0.094 & 0.001 & 0.001 & 0.001 & 0.094 & 0.000 & 0.001 & 0.000 & 0.050 & 0.000 & 0.001 & 0.001 & 0.082 \\
%irish & 0.000 & 0.002 & 0.000 & 0.20 & 0.000 & 0.001 & 0.000 & 0.21 & 0.000 & 0.001 & 0.000 & 0.092 & 0.000 & 0.001 & 0.000 & 0.14 \\
%kddcup & 0.002 & 0.032 & 0.003 & 9.54 & 0.002 & 0.007 & 0.002 & 5.69 & 0.003 & 0.045 & 0.011 & 31.00 & 0.005 & 0.010 & 0.006 & 16.17 \\
kr-vs-kp & 0.001 & 0.008 & 0.002 & 2.17 & 0.001 & 0.004 & 0.001 & 1.22 & 0.001 & 0.009 & 0.004 & 3.41 & 0.001 & 0.003 & 0.002 & 1.49 \\
lending & 0.001 & 0.003 & 0.001 & 1.99 & 0.001 & 0.003 & 0.001 & 1.51 & 0.004 & 0.030 & 0.006 & 9.13 & 0.008 & 0.039 & 0.010 & 15.99 \\
letter & 0.002 & 0.062 & 0.002 & 13.36 & 0.002 & 0.007 & 0.003 & 14.30 & 0.034 & 0.11 & 0.052 & 19.50 & 0.078 & 0.16 & 0.11 & 40.77 \\
lymphography & 0.001 & 0.007 & 0.002 & 0.32 & 0.001 & 0.003 & 0.001 & 0.20 & 0.000 & 0.002 & 0.001 & 0.13 & 0.001 & 0.001 & 0.001 & 0.090 \\
%messidor & 0.000 & 0.001 & 0.000 & 0.096 & 0.000 & 0.001 & 0.000 & 0.11 & 0.001 & 0.006 & 0.003 & 1.06 & 0.002 & 0.004 & 0.002 & 0.74 \\
%promoters & 0.000 & 0.001 & 0.001 & 0.063 & 0.000 & 0.001 & 0.000 & 0.053 & 0.000 & 0.002 & 0.000 & 0.046 & 0.000 & 0.001 & 0.000 & 0.045 \\
mushroom & 0.001 & 0.004 & 0.001 & 3.11 & 0.001 & 0.002 & 0.001 & 2.20 & 0.001 & 0.003 & 0.001 & 2.46 & 0.001 & 0.002 & 0.001 & 1.54 \\
%mux6 & 0.001 & 0.002 & 0.001 & 0.076 & 0.001 & 0.002 & 0.001 & 0.069 & 0.000 & 0.001 & 0.001 & 0.040 & 0.000 & 0.002 & 0.001 & 0.035 \\
%new-thyroid & 0.000 & 0.002 & 0.000 & 0.078 & 0.000 & 0.001 & 0.000 & 0.086 & 0.000 & 0.001 & 0.001 & 0.17 & 0.001 & 0.001 & 0.001 & 0.15 \\
pendigits & 0.002 & 0.063 & 0.003 & 10.03 & 0.002 & 0.007 & 0.003 & 8.45 & 0.008 & 0.047 & 0.011 & 37.59 & 0.015 & 0.056 & 0.019 & 61.59 \\
%postoperative & 0.001 & 0.002 & 0.001 & 0.093 & 0.001 & 0.002 & 0.001 & 0.077 & 0.000 & 0.002 & 0.001 & 0.048 & 0.000 & 0.002 & 0.001 & 0.040 \\
%primary-tumor & 0.001 & 0.005 & 0.002 & 0.47 & 0.001 & 0.004 & 0.001 & 0.28 & 0.001 & 0.001 & 0.001 & 0.17 & 0.001 & 0.001 & 0.001 & 0.13 \\
promoters & 0.000 & 0.000 & 0.000 & 0.017 & 0.000 & 0.000 & 0.000 & 0.024 & 0.000 & 0.001 & 0.000 & 0.039 & 0.000 & 0.001 & 0.000 & 0.037 \\
recidivism & 0.002 & 0.061 & 0.003 & 3.65 & 0.002 & 0.006 & 0.002 & 2.59 & 0.005 & 0.087 & 0.010 & 11.69 & 0.010 & 0.084 & 0.015 & 18.26 \\
%schizo & 0.000 & 0.002 & 0.001 & 0.22 & 0.000 & 0.001 & 0.001 & 0.17 & 0.001 & 0.003 & 0.002 & 0.58 & 0.001 & 0.002 & 0.001 & 0.37 \\
%segmentation & 0.000 & 0.001 & 0.000 & 0.098 & 0.000 & 0.001 & 0.000 & 0.096 & 0.001 & 0.002 & 0.001 & 0.30 & 0.001 & 0.002 & 0.001 & 0.25 \\
seismic\_bumps & 0.001 & 0.003 & 0.001 & 1.08 & 0.001 & 0.002 & 0.001 & 0.68 & 0.001 & 0.004 & 0.002 & 1.83 & 0.001 & 0.002 & 0.001 & 0.69 \\
shuttle & 0.001 & 0.006 & 0.001 & 22.65 & 0.001 & 0.005 & 0.001 & 22.35 & 0.002 & 0.061 & 0.002 & 2.85 & 0.003 & 0.060 & 0.003 & 3.56 \\
soybean & 0.001 & 0.058 & 0.002 & 1.17 & 0.001 & 0.005 & 0.001 & 0.82 & 0.001 & 0.005 & 0.003 & 1.65 & 0.001 & 0.003 & 0.002 & 0.95 \\
spambase & 0.001 & 0.008 & 0.003 & 3.43 & 0.001 & 0.003 & 0.001 & 1.81 & 0.002 & 0.069 & 0.009 & 11.20 & 0.003 & 0.062 & 0.003 & 4.18 \\
spect & 0.001 & 0.006 & 0.002 & 0.52 & 0.001 & 0.004 & 0.001 & 0.24 & 0.000 & 0.001 & 0.001 & 0.17 & 0.000 & 0.001 & 0.000 & 0.11 \\
splice & 0.000 & 0.001 & 0.000 & 0.22 & 0.000 & 0.002 & 0.000 & 0.30 & 0.001 & 0.064 & 0.002 & 1.48 & 0.003 & 0.069 & 0.004 & 3.43 \\
%student-mat & 0.002 & 0.061 & 0.003 & 1.14 & 0.002 & 0.007 & 0.002 & 0.92 & 0.002 & 0.058 & 0.005 & 1.98 & 0.003 & 0.060 & 0.004 & 1.56 \\
%student-por & 0.002 & 0.059 & 0.003 & 1.94 & 0.002 & 0.004 & 0.002 & 1.53 & 0.003 & 0.062 & 0.008 & 5.05 & 0.004 & 0.072 & 0.006 & 3.63 \\
%tram\_2000 & 0.000 & 0.001 & 0.000 & 0.10 & 0.000 & 0.001 & 0.000 & 0.15 & 0.000 & 0.001 & 0.000 & 0.10 & 0.000 & 0.001 & 0.000 & 0.15 \\
%uci\_mammo & 0.001 & 0.003 & 0.002 & 0.23 & 0.001 & 0.002 & 0.001 & 0.15 & 0.001 & 0.002 & 0.001 & 0.12 & 0.001 & 0.001 & 0.001 & 0.079 \\
%vehicle & 0.001 & 0.008 & 0.002 & 1.74 & 0.001 & 0.006 & 0.002 & 1.52 & 0.002 & 0.060 & 0.003 & 2.81 & 0.002 & 0.061 & 0.003 & 2.51 \\
%wdbc & 0.000 & 0.001 & 0.000 & 0.16 & 0.000 & 0.001 & 0.000 & 0.18 & 0.002 & 0.062 & 0.007 & 3.85 & 0.002 & 0.004 & 0.002 & 1.41 \\
%yeast & 0.001 & 0.002 & 0.001 & 0.33 & 0.001 & 0.002 & 0.001 & 0.42 & 0.004 & 0.10 & 0.007 & 3.06 & 0.008 & 0.072 & 0.011 & 5.04 \\

\bottomrule[1.2pt]
\end{tabular}
}
\end{adjustbox}
%\caption{\footnotesize{Assessing runtimes of the tree traversal
%    algorithm and the propositional horn encoding approach for
%    extracting one AXp.
%    %%Runtimes comparison between Traversal method and Horn encoding
%    %%method to extract one PI-explanation. 
%    %
%    The table reports the results for DTs trained with ITI and IAI
%    learning tools. Columns  {\bf m}, {\bf M} and  {\bf avg}  report,
%    resp.\ , the minimal, maximal and average runtime (in second)
%    to compute an AXp, while column {\bf Tot} reports the total
%    runtime (in second) of all tested instances in a dataset. } 
%\label{tab:runtime}}
\end{table}


==> texfigs/tree08.tex <==
\tikzset{every label/.style={xshift=-0.15ex,
  yshift=-6.15ex,
  text width=1ex,
  align=right, inner sep=1pt, font=\tiny, text=midblue}}
%
\tikzset{tlabel/.style={xshift=0.25ex, yshift=2ex, text width=1ex,
    align=right, inner sep=1pt, font=\tiny, text=midblue}}
%
\tikzset{EV/.style = {font=\scriptsize}}
%
\forestset{
  BDT/.style={
    for tree={
      %text=midblue,
      %l=1.125cm,s sep=1.0cm,
      l=1.5cm,s sep=1.25cm,
      if n children=0{}{circle},
      %draw=midblue,
      draw,
      edge={
        my edge
      },
      %if n=2{
      %  edge+={0 my edge},
      %}{},
      %font=\sffamily,
    }
  },
}
%
\begin{forest}
  BDT
  [$E$, %label={[yshift=0.425ex]1} %[xshift=0.125ex,yshift=-0.725ex]
    [$M$, %label={[yshift=-0.15ex]2}, %edge=very thick,
      edge label={node[EV,near start,left,xshift=-2.5pt] {$\in\{E_1\}$}}
      [$S$, %label={[yshift=0.425ex]4}, %edge=very thick,
        edge label={node[EV,near start,left,xshift=0pt] {$\in\{M_2\}$}}
        [{\footnotesize$\clyes$}, fill={tred3!20},
          edge label={node[EV,midway,left,xshift=-0pt] {$\in\{S_1\}$}}
        ]
        [{\footnotesize$\clnot$}, fill={tgreen3!25},
          edge label={node[EV,midway,right,xshift=0pt] {$\in\{S_2,S_3\}$}}
        ]
      ]
      [{\footnotesize$\clnot$}, fill={tgreen3!25},
        edge label={node[EV,near start,right,xshift=-0pt] {$\in\{M_1\}$}}
      ]
    ]
    [$M$, %label={[yshift=-0.15ex]3}, %edge=very thick,
      edge label={node[EV,near start,right,xshift=2pt] {$\in\{E_2,E_3\}$}}
      [$A$, %label={[yshift=-0.15ex]3}, %edge=very thick,
        edge label={node[EV,near start,left,xshift=0pt] {$\in\{M_2\}$}}
        %
        [$S$, %label={[yshift=0.425ex]6}, %[xshift=0.125ex,yshift=-0.725ex]%edge=very thick,
          edge label={node[EV,near start,left,xshift=-2pt] {$\in\{A_3\}$}}
          [{\footnotesize$\clyes$}, fill={tred3!20},
            edge label={node[EV,near start,left,xshift=0pt] {$\in\{S_1\}$}}
          ]
          [{\footnotesize$\clnot$}, fill={tgreen3!25},
            edge label={node[EV,near start,right,xshift=-0pt] {$\in\{S_2,S_3\}$}}
          ]
        ]
        [$S$,
          edge label={node[EV,near start,right,xshift=2pt] {$\in\{A_1,A_2\}$}}
          [{\footnotesize$\clyes$}, fill={tred3!20},
            edge label={node[EV,near start,left,xshift=0pt] {$\in\{S_1\}$}}
          ]
          [{\footnotesize$\clnot$}, fill={tgreen3!25},
            edge label={node[EV,near start,right,xshift=-0pt] {$\in\{S_2,S_3\}$}}
          ]
        ]
      ]
      %
      [{\footnotesize$\clnot$}, fill={tgreen3!25},
        edge label={node[EV,near start,right,xshift=-0pt] {$\in\{M_1\}$}}
      ]
    ]
  ]
\end{forest}

